Topology Guidance: Controlling the Outputs of Generative Models via Vector Field Topology

For domains that involve numerical simulation, it can be computationally expensive to run an ensemble of simulations spanning a parameter space of interest to a user. To this end, an attractive surrogate for simulation is the generative modeling of fields produced by an ensemble, allowing one to synthesize fields in a computationally cheap, yet accurate, manner. However, for the purposes of visual analysis, a limitation of generative models is their lack of control, as it is unclear what one should expect when sampling a field from a model. In this paper we study how to make generative models of fields more controllable, so that users can specify features of interest, in particular topological features, that they wish to see in the output. We propose topology guidance, a method for guiding the sampling process of a generative model, specifically a diffusion model, such that a topological description specified as input is satisfied in the generated output. Central to our method, we couple a coordinate-based neural network used to represent fields, with a diffusion model used for generation. We show how to use topologically-relevant signals provided by the coordinate-based network to help guide the denoising process of a diffusion model. This enables us to faithfully represent a user's specified topology, while ensuring that the output field remains within the generative data distribution. Specifically, we study 2D vector field topology, evaluating our method over an ensemble of fluid flows, where we show that generated vector fields faithfully adhere to the location, and type, of critical points over the spatial domain. We further show the benefits of our method in aiding the comparison of ensembles, allowing one to explore commonalities and differences in distributions along prescribed topological features.

==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by $Author: jpeltier $ $Date: 2007-04-03 16:51:34 -0700 (Tue, 03 Apr 2007) $
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers
according to the specifications for submission to conferences sponsored
by the IEEE Visualization & Graphics Technical Committee (VGTC). This
includes:

Conferences that use the 'conf' document option:
- IEEE Virtual Reality
- IEEE Symposium on 3D User Interfaces
- Symposium on Haptic Interfaces for Virtual Environment and Teleoperator Systems
- IEEE Symposium on Asia Pacific Visualisation
- IEEE Symposium on Interactive Ray Tracing
- IEEE Symposium on Visual Analytics Science and Technology
- IEEE Symposium on Visual Analytics Science and Technology
- IEEE Visualization Conference (Posters Only)
- IEEE Information Visualization Conference (Posters Only)
- IEEE Symposium on Volume Graphics

It contains 11 files/directories:

README          - this file
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default conference mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> sections-matt/methods.tex <==
\section{Methods}



% specifying a critical point: minimize vector norm (3~4
% -> this implies an energy function for diffusion guidance
% -> what is the input? a specified position in the domain
% -> boundary effects?
% -> guidance strength
% -> time steps at which to introduce guidance

% forward guidance

% paragraph: different types of critical points ~3
% -> definition of critical point
% -> how we formulate this as an energy for diffusion guidance
% 1. we can get closed form of eigenvalues from INR 2. sigmoid function to classify

% paragraph 
% -> trade-off between specifying the presence of a critical point & type of critical point
% -> does the type guidance make sense if, at this location, no critical point exists? (line plot with the reverse diffusion)

% paragraph: stable vs. unstable
% -> definition
% -> accessing this from the INR
% -> energy function

% paragraph: combination
% composing energy functions: type + stability

% paragraph: multiple critical points
% composition of everything

==> sections/introduction.tex <==
% paragraph 1 : motivate the use of generative models for numerical simulations
% Problem 1: understanding physical phenomena is limited by the compuation resources we have to run numerical simulations
% Solution 1: generative models can help us "fill in the gaps" -> we build generative models over the outputs of numerical simulations; in turn, if we want to study an output, we just need to sample from the generative model -> this becomes a surrogate for a numerical simulation
Through the use of advanced computer simulations, simulation based on PDE is widely used for the exploration of intricate real-world phenomena.
Due to the physical phenomena being studied often has a natural uncertainty,
a single run with a group of freezing parameter is not adequate.
As a result, domain experts execute multiple runs across a large parameter space, including the initial conditions, boundary and adjustable input parameters. The generated data is called ensemble simulation data.
However, the execution of multi simulations is notably resource-intensive, presenting a significant barrier due to the high computational costs and I/O bottleneck associated with multiple runs.
Given this context, applying deep learning techniques to generate ensemble simulation data across a broad parameter space has the potential to mitigate the computational expenses traditionally associated with ensemble simulations. 
This solution offer a powerful approach to augment the outputs of numerical simulations by generating plausible samples. 
By constructing generative models over the simulation outputs, we can effectively "fill in the gaps" and alleviate the need to rerun the computationally intensive simulations whenever we wish to study specific output configurations. 
The generative model serves as an efficient surrogate for the original simulations, allowing us to sample from its learned distribution to obtain realistic instances of the physical phenomena.

% paragraph 2 : the problem -> how do we make useful for end users?
% Problem 2: you don't know what you are going to get when you sample from a generative model; we need more intuitive, and more controllable, methods for sampling from generative models when we want to explore a distribution of fields
% What does intuitive mean?
    % What kinds of features are relevant to domain scientists when studying fields produced in numerical simulations?
% TOPOLOGY.
% How do we make generation more informed by the features people care about?
However, generating useful and intuitive samples from simulation generative models for end-users remains a challenge.
Domain experts need to explore the property of the field with the understand of topological features, such as fixed points (sources, sinks, and saddles) and periodic orbits, which have been studied extensively in the context of steady flow\cite{}.
Fixed points, such as sources, sinks, and saddles, play a crucial role in the analysis of fields, as they provide valuable insights into the governing dynamics of the surrounding fluid, enabling experts to trace the origin (source) and destination (sink) of particles within the domain. Domain experts can explore and understand the underlying dynamics and patterns with such topological features.
In addition, to make generative models more applicable and accessible to end-users, it is crucial to develop sampling methods that are not only more intuitive but also offer greater control over the sampling process, allowing users to focus on the features that are most relevant to their analysis.
By integrating domain-specific constraints, such as topological information, into the sampling process, we can create more informed and controllable generative models that align with the needs and expectations of domain experts, ultimately facilitating the exploration and understanding of complex field distributions from numerical simulations.
A generative model without any control require the users to sample over and over again until they get the result they want. This could be worse for simulation data generation due to the need of additional rendering pipeline for field visual analytics, which is both time and resource consuming. 

% paragraph 3 : our approach - high level
We propose Topology Guidance, a method that augments the field sampling process of a generative model by incorporating topological constraints without requiring additional network training.
This topology guidance is valuable for two key reasons.
First, while the sampling results of generative models are typically in-distribution, the specific features of the generated fields may not always align with the user's desired output. By introducing topological constraints during the sampling process, users gain control over the model's output, ensuring that it generates fields with the topological structures they are interested in, without the need for repeated trial and error.
Second, the samples generated by Topology Guidance belong to a specific ensemble simulation with a broad parameter configuration. As a result, the fields generated with certain topological structures can be considered as data augmentation for the simulation.
Topology Guidance thus provides a powerful and efficient way for domain experts to explore and analyze large-scale fluid flow fields simulation data distribution.

% paragraph 4 : technical contributions
To address the challenges posed by the multi-dimensional and high-dimensional nature of simulation data, which often requires substantial computational resources, we first convert the high-dimensional simulation data to low-dimensional data parameterized by a simple network architecture [cite].
This data pre-processing approach compresses the large-scale ensemble data and reduces the disk resources required for modeling the ensemble data distribution, enabling its incorporation with a generative model for subsequent exploration. We then train the generative model directly in this latent space.
Our generative model is based on the Denoising Diffusion Probabilistic Models [cite], which focuses on probabilistically removing noise from data. During training, the model learns how noise is added to data over time and how to reverse this process to recover the original data.
We leverage this off-the-shelf denoiser to guide the sample towards a specific direction during the denoising process, with the direction being the user-specified topological constraints.
The key challenge lies in finding the sweet spot that allows the sampling to adhere to the topological constraints while maintaining the realness of the generated fields. To trade off between these, we apply the forward topology guidance[cite], which ensures that the sampled field moves off the manifold less than the denoiser can correct, resulting in the final sample being within the ensemble data distribution.

% paragraph 5 : experimental evaluation

% paragraph 6 : summary with bullet points
To sum up, we make the following contributions:
\begin{enumerate}
    \item We propose Topology Guidance - a method that enhances the sampling process of generative models by incorporating user-specified topological constraints, enabling the generation of fields with desired features while maintaining their realness. This method can also provide an efficient way for domain experts to explore and analyze ensemble simulation data distributions.
    \item We evaluate the proposed method on a subset of 8,000 unsteady 2D vector fields, each with a resolution of 512 × 512 voxels and 1001 time steps, amounting to a total of 16 TB.
We extract its latent representation and train a diffusion model in the low-dimensional space. 
Topology guidance is used to control the 2D vector fields generation. Both qualitative and quantitative results show that we are able to generate 2D vector fields that follow the specified topology constraints as well as are in original data distribution.
\end{enumerate}

% The topology structure of vector field has seen widespread applications since its introduction to visualization by Helman and Hesselink\cite{helmanRepresentationDisplayVector1989} more than 30 years ago.
% One of the topology structures being explored is critical points because it can indicate where the vector field vanishes, e.g., the velocity at that point is 0.
% In order to have a deeper insights of a ensemble simulation dataset,
% domain experts need to have a better understanding of the topology distribution, for instance,
% how likely there would exist a saddle point on the top left of the vector field.
% To quantify this probability, there are existing work exploring the critical points extraction supporting both the position and the type  of the point, but these methods can only be applied to a single data point with one parameter configuration.
% Since the ensemble vector field dataset usually has a large simulation parameters space,
% domain users have to conduct the topology structure extraction algorithms for multiple times to understand the topology distribution.
% Another research gap is that it is hard to save all the raw ensemble data for post hoc data summarization and analysis.

==> sections/methods.tex <==
In this section we present our approach for topology guidance, namely, how to guide a diffusion model of vector fields towards a user-specified topology configuration. We organize topology guidance along the following factors:
\begin{enumerate}
    \item \textbf{Critical point}: ensuring that a critical point exists at a specified location.
    \item \textbf{Type of critical point}: distinguishing a critical point whether it is attracting, repelling, or a saddle.
    \item \textbf{Stability of a critical point}: attracting \& repelling critical points can be further categorized as stable, or unstable.
\end{enumerate}
A key aspect of our approach is the \emph{composition} of the above factors, e.g. a user may wish to study a distribution of fields that merely have some type of critical point at a given location; alternatively, they may be highly precise in their specification.
We discuss each of these factors step by step, namely, how to derive suitable guidance functions (c.f. Sec.~\ref{}).

\subsection{Prescribing a critical point}

The most general form of guidance is simply specifying that a critical point exists at a given location.
A critical point is defined as a location in the field whose vector components are all zero.
This can equivalently be phrased as the vector's norm being zero at the location.
Thus, we can derive a suitable guidance function by prescribing that the norm of the vector field should be minimized at a given location:
\begin{equation}
    \mathcal{E}_c(\mathbf{z}_t , t; C) = \lVert f_{\phi}(\mathbf{p} ; \mathbf{z}_t) \rVert,
\end{equation}
where $C = (\mathbf{p})$ contains the location $\mathbf{p} \in \mathbb{R}^2$ in the domain where the user intends to introduce a critical point.

The key idea behind presence guidance is to minimize the vector norm at the specified critical point locations. 
This approach is inspired by the definition of a critical point in a vector field, which states that a critical point is a position where the vector norm equals zero, as shown in ~\cref{fig:methods-guidance}(1):
\begin{equation}
    \|v(x,y)\|=0.
\end{equation} 

\begin{figure}[htbp]
    \centering
    \includegraphics[width=1\linewidth]{images/methods_guidance.pdf}
    \caption{Guidance description}
    \label{fig:methods-guidance}
\end{figure}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=1\linewidth]{images/methods_energy.pdf}
    \caption{Illustration of the manipulation of the logits.}
    \label{fig:methods-energy}
\end{figure}

By explicitly minimizing the vector norm at the desired critical point locations, \textit{Presence Guidance} encourages the diffusion model to generate vector fields that exhibit the specified critical point behavior. 
To implement this solution, we design an energy function used for guidance. 
The energy function takes as input a specified position in the domain and aims to minimize the vector norm at that location. The specific form of the energy function is given by:
\begin{equation}
    E(x)=\|v(x,y)\|\text{,}
\end{equation}
where $v(x,y)$ represents the vector at position $(x,y)$ in the generated vector field.

When designing the energy function for presence guidance, several important parameters and considerations need to be taken into account. Firstly, boundary effects are not considered in the energy function since critical points are difficult to define near the boundaries of the domain. 
Secondly, the guidance strength is a crucial parameter that determines the balance between fidelity to the original diffusion model and adherence to the critical point constraints. If the guidance strength is too high, it may compromise the overall fidelity of the generated vector field. Conversely, if the guidance strength is too low, the critical point constraints may not be sufficiently followed. 
Through empirical experiments, an appropriate value for the guidance strength is selected to strike a balance between these competing objectives. 

Another important aspect is the choice of time steps at which to introduce the guidance. Since the denoising process starts from random noise, the initial steps of the diffusion model may produce highly distorted samples. Therefore, it is not desirable to introduce guidance too early in the process. 
On the other hand, introducing guidance too late may be ineffective because the local behavior of the sample has already formed and becomes difficult to modify. 
A carefully chosen threshold is determined for introducing the guidance, based on the observation that the vector norm starts to decrease and gradually approaches zero at a certain point during the denoising process, as shown in ~\cref{fig:methods-norm}. 

\begin{figure}[htbp]
    \centering
    \includegraphics[width=1\linewidth]{images/methods_norm.pdf}
    \caption{Enter Caption}
    \label{fig:methods-norm}
\end{figure}

It is worth noting that the diffusion model is trained on clean vector fields. 
Simply compute the energy function conditioned on each $z_t$ may not provide useful guidance. 
The denoising process may sacrifice stability to meet constraints because it moves towards the direction of the guidance constraints faster than the denoiser guides towards the data space.
Reducing the scaling factor $s$ could enforce the sampling go towards the data space, but it would also fail to meet the guidance constraints. 
To address this, the energy function is applied in the predicted clean space, as introduced in~\cref{eq:DDIM}. 
In summary, the sampling process incorporated with our energy function to prescribe the critical point shown in ~\cref{alg:sample}.
\begin{algorithm}[H]
\caption{Topology Guidance during Sampling Process}
\label{alg:sample}
\begin{algorithmic}[1]
\Statex \textbf{Input}: Topology specification \textbf{$c$}
\Statex \textbf{Output}: Data distribution with the specified topology \textbf{$z$}
\State $z_T \sim \mathcal{N}(0, I)$
\For{$t = T, ..., 1$} 
    \State $\epsilon \sim \mathcal{N}(0, I)$ if $t > 1$, else $\epsilon = 0$ 
    \State $\tilde{\epsilon}_{\theta}(x_t, t) = \epsilon_{\theta}(x_t, t) + s\nabla_{\hat{z_t}}\mathcal{L}(c,f(\hat{z_0})) $
    \State $z_{t-1} = \frac{1}{\sqrt{\alpha_t}} \left( z_t - \frac{1-\alpha_t}{\sqrt{1-\alpha_t}} \tilde{\epsilon}_{\theta}(z_t, t) \right) + \sigma_t \epsilon$ 
\EndFor
\State \Return $z_0$
\end{algorithmic}
\end{algorithm}

\textbf{Type Guidance}. 
Type Guidance builds upon Presence Guidance by generating critical points at specified locations while also specifying their type. Critical point types, namely sinks, sources, and saddles, are defined by the eigenvalues $\lambda_1,\lambda_2$ of the Jacobian matrix $J$, which characterizes the local behavior of a vector field around a critical point. 
\begin{equation}
J(\lambda_1, \lambda_2) =
\begin{cases}
\text{Sink},  & \lambda_1 < \lambda_2 < 0\\
\text{Source}, & 0 < \lambda_1 < \lambda_2 \\
\text{Saddle}, & \lambda_1 < 0 < \lambda_2
\end{cases}    
\end{equation}
To formulate this as an energy for diffusion guidance, we can obtain closed-form expressions for the eigenvalues from a coordinate-based neural network. Given a vector field $(u,v)$ at a point $(x,y)$, the Jacobian is a $2\times2$ matrix of partial derivatives: 
\begin{equation}
J=
\begin{bmatrix}
\frac{\partial x}{\partial u} & \frac{\partial x}{\partial v} \\
\frac{\partial y}{\partial u} & \frac{\partial y}{\partial v}
\end{bmatrix},
\end{equation}
And from this, we can further derive the exact eigenvalues of the Jacobian matrix.

Drawing inspiration from activation functions in neural networks, we employ a sigmoid function for classification. The sigmoid controls the sign of the Jacobian matrix's eigenvalues, thereby controlling the type of critical point. For instance, if both eigenvalues are currently positive but we desire to sample a sink, we apply the function:
\begin{equation}
    E=\sigma(x)=\frac{1}{1+e^x}. 
\end{equation}
Likewise, if both eigenvalues are currently negative but we desire to sample a source, we apply the function:
\begin{equation}
    E=\sigma(x)=\frac{1}{1+e^{-x}}.
\end{equation}
Since the energy function serves as a loss function, its value is continually minimized, driving the logit towards 0, as illustrated in the ~\cref{fig:methods-energy}.

%TODO justify the tradeoffs

\textbf{Spirality Guidance}. It extends the concept of Type Guidance by distinguishing spiral attributes of either sink or source. For a 2x2 Jacobian matrix, its determinant is denoted as $Det$, and its trace is denoted as $Tr$. 
We define the discriminant as $\Delta=Tr^2 - 4Det$. 
The spirality of a critical point depends on the sign of the discriminant. 
When $\Delta < 0$, the eigenvalues are complex numbers. In this case, if $Tr < 0$, the critical point is a stable spiral sink; if $Tr > 0$, the critical point is an unstable spiral source.

To obtain stability information from the coordinate-based neural network, we can compute the determinant, trace, and discriminant of the Jacobian matrix at each critical point location. By evaluating these quantities, we can determine the stability of the critical point. When incorporating Stability Guidance into the energy function, we can also extend the sigmoid-based classification approach used in Type Guidance. 
For example, to encourage the generation of a spiral point, we can design an energy function:
\begin{equation}
    E = \sigma(\Delta)=\frac{1}{1+e^{\Delta}}, 
\end{equation}
where $\sigma$ is the sigmoid function. 
By minimizing this energy function during the diffusion process, the network learns to generate vector fields with stable spiral sinks at the desired locations.

\textbf{Combination of Guidance}. 
To achieve finer control over the generated vector fields, we can combine Type Guidance and Spirality Guidance by simultaneously controlling both the type and spirality of the critical points. This is accomplished by composing the energy functions for type and spirality using a linear combination:

The linear combination of energy functions is effective because it allows for a balanced influence of both type and spirality constraints on the denoising process. By adjusting the weights of each energy term, we can prioritize one aspect over the other or give them equal importance. This flexibility enables us to generate a wide range of vector field patterns with desired characteristics. For instance, to generate a stable spiral sink, we can combine the energy functions for a sink and a spiral:
\begin{equation}
    E = w_\text{type} \cdot E_\text{sink} + w_\text{spirality} \cdot E_\text{spiral},    
\end{equation}
where $w_\text{type}$ and $w_\text{spirality}$ are the weights assigned to the type and spirality energy terms, respectively. The sink energy term $E_\text{sink}$ encourages the eigenvalues to be negative, while the stable spiral energy term $E_\text{spiral}$ pursues a negative discriminant.

\textbf{Multiple Critical Points}.
%TODO add more descriptions
The linear combination of energy functions is a simple yet effective approach to composing multiple constraints for guiding the diffusion process. 


==> sections/relatedwork.tex <==
\section{Related Work}

Our work broadly fits 

\subsection{Deep Learning for Ensemble Data}
% para 1
% related: Deep learning based latent representations
Based on the data type (scalar field or vector field, time-dependent or time-independent) and the specific deep learning task, researchers often carefully select the inputs and outputs of the neural network .
To generate volume data, the input of neural network usually is low-resolution version of data~\cite{TSR-TVD}, voxel coordinate~\cite{neurcomp}, simulation parameters~\cite{GNN-surrogate} and field volume~\cite{scalar2vec}, and the output could be super-resolution version of data, scalar or vector value, field feature (density or color).
% network architecture: CNN, GNN, GCN, AE (ours)

% para 2
% gap: unsupervised learning has better generalizability
The DL task can be categorized into supervised, semi-supervised, and unsupervised\cite{jingSelfsupervisedVisualFeature2019}.
Medical imaging, for example, requires expert annotations, which are time-consuming and costly to obtain.
Volume data is inherently high-dimensional, with each voxel representing a point in 3D space. This high dimensionality poses computational challenges, as deep learning models need to process and generate large amounts of data, leading to increased memory requirements and slower training and inference times.
The definition of INR is to represent complex data such as audio, images, and 3D scenes as implicit continuous functions through parameterized Multilayer Layer Perceptrons (MLPs). 
Due to the slow convergence rate of standard MLPs, Tancik et al. improved the INR's performance in learning high-frequency functions by simply applying a Fourier feature mapping to the network's inputs. 
Similarly, Sitzmann et al.\cite{sitzmannImplicitNeuralRepresentations2020} proposed the use of sinusoidal representation networks (SIREN) with periodic activation functions in INRs. 
This method accurately models the temporal and spatial derivatives of simulation data implicitly defined by differential equations.
%latent representation and modulation
Applying INR to volume visualization offers significant benefits. 
When analyzing ensemble data generated from simulations, the vast simulation parameter space necessitates multiple simulation runs, each resulting a different data instance. 
As such simulation runs generate a giant amount of data, often ranging from tens to hundreds of GB, loading such large datasets into memory for visual analysis via a personal computer's I/O bandwidth becomes impractical.
In this context, INR provides an efficient solution, particularly in terms of volume data compression. 
Lu et al. demonstrates a method for representing scalar fields as learned functions, where adjusting the weights of a neural network can achieve compressed data representation. This method is especially effective when the number of network weights is less than the size of the input data. Moreover, it supports compression of time-varying scalar fields and allows for random access evaluation of the field, outperforming current state-of-the-art techniques in volume data compression.
CoordNet\cite{hanCoordNetDataGeneration2023} is also a coordinate-based framework, decomposing diverse task inputs and outputs into a unified representation (i.e., coordinates and values) and learn a function from coordinates to their corresponding values.
However, even with a minor change of the data instance, it is necessary to retrain an INR. 
A shared, pre-computed initialization has been advocated as a good practice when fitting INRs, e.g., to reduce training time by means of meta-learned initialization vectors~\cite{inr2vec, functa}.
Jiao et al. proposed Feature-Enhanced Implicit Neural Representation (FFEINR) for spatio-temporal super-resolution of flow field data.


\subsection{Surrogate Models for Ensemble Data}
\label{relatedwork-surrogate}
% para 1
Unlike traditional rendering pipelines, some existing work directly generate previously unseen visualization results according to the given input parameters, without requiring re-running simulations under new parameter settings. Instead, they .
Recent years, researchers treat this topic also as the surrogate model for volumetric data.
Existing work have explored how to improve the accuracy and efficiency of fluid simulation by replace traditional numerical solvers with learned solvers~\cite{Transformers for modeling physical systems,Predicting physics in mesh-reduced space with temporal attention,Learned coarse models for efficient turbulence simulation,Latent space physics: Towards learning the temporal evolution of fluid flow}.
Moreover, in order to predict simulation data that maintain both stability and accuracy, Kohl~\cite{Benchmarking Autoregressive Conditional Diffusion Models for Turbulent Flow Simulation} proposed a probabilistic surrogate flow simulator, representing state of the art diffusion models applied to flow prediction.
Existing generative models focus more on conditioning on specific physical properties and simulation parameters, such as Reynolds number, time step, etc., to predict flows that comply with physical prior knowledge. 
%TODO, adress the similarity between Computer vision and scivis, then introduce the guided diffusion
However, the sampling process of generative models is expensive.
In addition, simulation data generation is not what you see is what you get; after generating the field, an explicit rendering pipeline is required for researchers to determine the visual characteristics of the generated data. 
Due to the above two challenges,
it costs for the researchers utilize the generative model as a surrogate simulator to generate a field with a specific visual characteristics (for example, generate a field vanishing on the left top), 
because they need to iteratively sample, render, and review the results until they generate the data point they want, which is both time and resource consuming. 
% Therefore, we propose a method that integrate the visual characteristics of the field as guidance into the generation process. 
% Experts can easily guide the generative model to produce flow fields with specific visual characteristics through such feature guidance.

% para 2
% gap: ours is unconditional
DNN-VolVis~\cite{hongDNNVolVisInteractiveVolume2019} can `reverse' the volumetric images interactively `reversed' given viewpoint.
Another approach~\cite{bergerGenerativeModelVolume2019} used the Generative Adversarial Network (GAN) framework to compute a conditional model with viewpoint and transfer function for opacity and color.
InSituNet\cite{heInSituNetDeepImage2019} is a convolutional regression model that enables flexible exploration of parameter spaces for large-scale ensemble simulations, by learning the mapping from simulation and visualization parameters to results, thereby overcoming the limitations of in situ visualization.
Similarly, Soumya et al.\cite{duttaSituDistributionGuided2017}introduces an in situ distribution guided stall analysis technique that utilizes probabilistic data modeling to efficiently summarize simulation data.
% importance-driven methods
Kunhua et al.\cite{suImportanceGuidedStream2023} proposed a novel surface generation and exploration scheme for the steady flow field, guided by a userspecified importance field. But it required explicit query or prior knowledge of the constraint. 
% unfold it with more details
IDLat introduced\cite{shenIDLatImportanceDrivenLatent2022} a novel approach for scientific data visualization and analysis that leverages spatial importance maps and a feature transformation network for domain-interest-guided latent representation generation

